A Quality Assessment Instrument for Systematic Literature Reviews in Software Engineering

Context: Systematic literature reviews (SLRs) have become standard practise as part of software engineering research, although their quality varies. To build on the reviews, both for future research and industry practice, they need to be of high quality. Objective: To assess the quality of SLRs in software engineering, we put forward an appraisal instrument for SLRs. The instrument is intended for use by appraisers of reviews, but authors may also use it as a checklist when designing and documenting their reviews. Method: A well-established appraisal instrument from research in healthcare was used as a starting point to develop a quality assessment instrument. It is adapted to software engineering using guidelines, checklists, and experiences from software engineering. As a validation step, the first version was reviewed by four external experts on SLRs in software engineering and updated based on their feedback. Results: The outcome of the research is an appraisal instrument for the quality assessment of SLRs in software engineering. The instrument intends to support the appraiser in assessing the quality of an SLR. The instrument includes 16 items with different options to capture the quality. The item is assessed on a two or three-grade scale, depending on the item. The instrument also supports consolidating the items into groups, which are then used to assess the overall quality of a systematic literature review. Conclusion: It is concluded that the presented instrument may be helpful support for an appraiser in assessing the quality of SLRs in software engineering.

==> Critical appraisal of SE SLRs (Paper)(1)/Guidance.tex <==
\newpage\clearpage
\onecolumn
\section*{Appendix B. QAISER Guidance Document}
\label{AppendixB}
In this document, we provide further guidance to support a consistent interpretation of items in QAISER.
\newline 

\noindent \textbf{Item 1: Did the authors of the review adequately justify the need for undertaking the review?}
\newline
A large number of SLRs are reported in software engineering every year. A review should be initiated on the basis of a practical or scientific need. The authors of the review should also extensively search for any existing reviews or mapping studies on the topic. The authors should only continue planning the review if there are no existing ones that are up to date on the specific area \cite{kitchenham2015evidence}. Mendes et al. \cite{MendesWFK20} provide support to decide if a review should be updated.

To score 'Partial Yes', appraisers should check if the authors of the view have made a sufficiently extensive effort to identify related reviews on the topic.  

To score 'Yes', appraisers should ensure that the authors of the review have established the need for undertaking the review. If there are existing reviews on the same topic, the authors need to establish the need by highlighting the gap in the existing reviews, and explaining how their review is going to fill the gap. In case there are no existing reviews on the topic, the authors explain why is it essential to aggregate the evidence on the topic.

The information about the need for review is typically described in the background or related work sections of the report.
\newline

\noindent \textbf{Item 2:	Did the authors of the review establish a protocol prior to the conduct of the review?}
To reduce the risk of bias, it is important that the authors of the review have developed and validated a written protocol before commencing the review. 

To score 'Partial Yes', appraisers should first check that the protocol is accessible and the review report describes where and how can it be accessed. Furthermore, the protocol should have documented appropriate review questions, the processes for search, study selection, data extraction, quality assessment and at least an outline for the data synthesis plan. 

To rate 'Yes', the protocol should have been validated both internally and by an independent reviewer and the authors of the review should have clearly documented and justified any deviations from the protocol and discuss their impact on the study. If the appraisers notice that the review report contains unexplained deviations from the protocol, they should downgrade the rating. 

The above information about the protocol is typically described in the methodology section of the review report. \newline

\noindent \textbf{Item 3:	Are the review's inclusion and exclusion criteria appropriate?}
A review should use documented selection criteria \cite{AMPATZOGLOU2019201,Sheaj4008,kitchenham2015evidence,PETERSEN20151,DARE}.

To score 'Yes', appraisers should ensure that the authors of the review have justified any restrictions, e.g., on research designs, the time frame of publication, and the type of publications imposed in the selection process. Furthermore, the justification should also address the likely impact of the restrictions on the studied population and the generalization of the findings. 

The selection criteria and the justifications for any restrictions are expected to be found in the methodology or limitations/threats to the validity section of the review report. Furthermore, some of the exclusion criteria may have been implemented in the search process.
\newline

\noindent \textbf{Item 4:	Did the authors of the review use a comprehensive literature search strategy?}
A comprehensive search strategy is important to maximize the coverage of the relevant literature. The authors of the review should provide a justification for using a particular search method (e.g., database or indexing service search or snowballing) as a primary method for searching the relevant literature. 

To rate 'Partial Yes', appraisers should check the following in case of a database or indexing service search as the primary search method:
\begin{itemize}
    \item The authors of the review have validated their search process by comparing their search results with a known-set of papers. The known-set of papers are the relevant papers that are already known to the authors of the review based on, for example, manual search or their knowledge of the review topic. The validation is performed by computing recall and precision using the search results and the known set of relevant papers (for details, refer to \cite{kitchenham2015evidence}).
    \item The authors of the review have used an appropriate process for identifying the search terms, synonyms and constructing the search strings.
    \item The authors of the review have used a combination of publisher databases and indexing services. IEEE and ACM are the most relevant publisher databases in software engineering, as they publish the most important and relevant conferences and journals in software engineering \cite{kitchenham2015evidence}. As a minimum, the authors should have used IEEE and ACM among the publisher databases and one indexing service (e.g. Scopus).
    \item The authors of the review have documented the search process. Appropriate documentation of the search process is important to ensure repeatability and transparency. The authors of the review should document: general and database specific search strings, total and database specific search results, search filters (e.g., years) used, date when the search strings were applied, known-set of papers used for validation, and validation measures (i.e. recall and precision) for details see \cite{AliU18}. 
    \end{itemize}
To rate 'Yes', the authors of the review should have also used at least one additional search method (e.g., snowballing).

To rate 'Partial Yes', appraisers should check the following in case of a snowballing search as the primary search method:
\begin{itemize}
     \item The authors of the review have used an appropriate process for identifying the seed set for starting the snowballing procedure. The way of identifying the seed set is well-documented and -motivated.
     \item The authors have iterated the snowballing procedure until no more papers are found.
     \item The authors of the review have validated their search process by comparing their search results with a known-set of papers. The known-set of papers are the relevant papers that are already known to the authors of the review based on, for example, manual search or their knowledge of the review topic. The validation is performed by computing recall and precision using the search results and the known set of relevant papers (for details, refer to \cite{kitchenham2015evidence}).
    \item The authors of the review have documented the search process. Appropriate documentation of the search process is important to ensure repeatability and transparency. The authors of the review should document: identification of the seed set, the different iterations conducted, known-set of papers used for validation, and validation measures (i.e., recall and precision). 
    \end{itemize}
To rate 'Yes', the authors of the review should have also used at least one additional search method (e.g., manual search of key journals or conference proceedings, or use DBLP or Google scholar of key researchers) or continuing snowballing iterations until no new papers are found).
\newline

\noindent \textbf{Item 5. Did the authors of the review use a reliable study selection process? }
To reduce bias and the possibility of making mistakes, the crucial step of inclusion and exclusion of the papers should involve at least two reviewers~\cite{AliP14,Sheaj4008}.

To rate 'Partial Yes', appraisers should check if at least two authors of the review selected a representative sample of eligible studies and achieved good agreement, with the remainder selected by one review author. A single reviewer should only proceed with the selection after a Kappa score indicating strong agreement between multiple authors of the review has been reached.

To rate 'Yes', appraisers should check that one of the two following processes are followed during study selection: 1) two authors of the review independently performed study selection on all eligible studies, reached consensus and also reported the agreement level, 2) two authors of the review selected a sample of eligible studies, achieved good agreement level, with the remainder selected by one review author, but in that case all excluded studies must be reviewed by at least two authors of the review. A single reviewer should only proceed with the selection after a Kappa score indicating strong agreement between multiple authors of the review has been reached. However, even in this case, the excluded studies should be reviewed by other authors of the review as well. Appraisers should also check that the rules for inclusion and exclusion, and how these rules were applied and how any differences between reviewers were resolved are described. Furthermore, the report should also report the number of papers remaining at each stage~\cite{BudgenBDW18}.

The information about the study selection process is expected to be described in the methodology and results sections of the review.
\newline

\noindent \textbf{Item 6.	Did the authors of the review use a reliable data extraction process?}
To ensure repeatability of the study and to avoid bias, it is important that the data extraction is not solely performed by a single researcher.

To rate 'Partial Yes', appraisers should check if the authors have performed pilot extraction of data on a sample of the included studies to develop a shared understanding of the data extraction form. 

To rate 'Yes', appraisers should ensure that data is extracted by at least two authors of the review either from all included studies OR from at least a sample of included studies. It is important to check that the review report provides a description of the mechanism used to achieve consensus and shared understanding on which data to collect.

The information of the data extraction process is generally described in the methodology section of the review report.
\newline

\noindent \textbf{Item 7:	Did the authors of the review provide a list of excluded studies, along with the justifications for exclusion, that were read in full text?}
This item refers to studies that were deemed relevant by authors of the review on a reading of the title and abstracts. However, after full-text reading, the authors concluded that the papers are not relevant to the current review. It is expected that the authors of the review should document such papers along with the reason for their exclusion. This will help increase confidence in the results, allow reflecting on the selection criteria used in the study, allow replications, and enable further research (for example, by leveraging on the filtered list of papers for a different analysis).

To rate 'Partial Yes', appraisers should see that the authors of the review have provided a list of such potentially relevant papers. In order to rate 'Yes', justifications for excluding the potentially relevant papers should also be provided. 

This documentation (i.e., a list of potentially relevant papers that were excluded after full-text reading and justifications for excluding them) can be made available in an appendix or as supplementary material for review online (along with other supporting material like the review's protocol).
\newline

\noindent \textbf{Item 8:	Did the authors of the review provide sufficient primary studies’ characteristics to interpret the results?}
The relevance and reliability of a systematic review depends, besides other factors, also on a number of factors related to the included studies such as its type (e.g., case study, survey, and experiment), context (real life or laboratory setting), participants (practitioners or students), and publication venue (e.g., a reputable conference/journal). The review report should describe adequate details about the characteristics of the included studies to inform the review readers about the kind of evidence that is used to draw conclusions.

To rate 'Yes', appraisers should ensure that the authors of the review have provided enough details about the population, interventions (when relevant), outcomes (when relevant), research designs and settings of the included studies.

These details may not be described at one place in a review report, and therefore could be challenging to find. Normally, part of this information is described in the start of the results section in a review report.
\newline

\noindent \textbf{Item 9:	 Did the authors of the review use an appropriate instrument for assessing the quality of primary studies that were included in the review?}
Due to several reasons, including the variety of research designs used in primary studies, reporting quality, use of inconsistent terminology, etc., quality assessment is a challenging task in software engineering systematic literature reviews \cite{kitchenham2015evidence,KITCHENHAM20132049}. Several research-design specific checklists (e.g. for experimentation~\cite{wohlin2012experimentation} and case study research \cite{host2007checklists}) and generic instruments (e.g. \cite{Wieringa12,condori2012experimental}) have been proposed in literature. However, as concluded by Kitchenham \cite{kitchenham2015evidence}, it is not feasible to use the same instrument to assess the quality of different types of studies.

To rate 'Yes', appraiser should ensure that the choice of the instruments used (whether an existing one or one formulated by the authors of the review) has been justified given the goals of the SLR and nature of included studies. Furthermore, the instrument used is expected to evaluate at least the research design, data collection, analysis reporting, and the strength of evidence given the stated goals of the primary study.

The information on the quality assessment of the primary studies is expected to be described in the methodology and results sections of the review report.
\newline

\noindent \textbf{Item 10:	Did the authors of the review use a reliable quality assessment process?}
Like Item 5 and 6, it is important that the quality assessment is not performed solely by a single author of the review.

To rate 'Partial Yes', appraisers should check if at least two authors have performed pilot quality assessment of a sample of the included studies to evaluate the objectivity of the quality assessment criteria and to develop a shared understanding of it. 

To rate 'Yes', appraisers should see that at least two authors of the review independently performed the quality assessment of either all included studies or a sample of included studies (with the remaining performed by one review author) and achieved good consensus. The review report should also describe how differences were resolved in case of different quality scores.

The information about the quality assessment process is typically expected in the methodology section of the review report.
\newline

\noindent \textbf{Item 11:	Were the primary studies appropriately synthesized?}
Synthesis is one of the most important and also challenging parts of a systematic literature review. Without synthesis, the review would be of limited use.

In order to score 'Yes', appraisers need to see if the authors of the review have used and justified an appropriate method for synthesis. It may be the case that the authors of the review do not use the correct or appropriate name for the used synthesis method \cite{CRUZES2011440}. In that case, appraisers would have to carefully read the review report in order to make a decision on this item. The appraisers should further check if the selected synthesis method was appropriately applied and that there is a clear chain of evidence from the answers to the research questions to the data from the primary studies.

The information about the synthesis method and its output may be documented in a separate section. In some cases it may be described in the discussion section after the results section. It could also be the case that the justification for selecting a specific synthesis method is described in the research methodology section, while the outputs of the synthesis step are described in a separate section. 
\newline

\noindent \textbf{Item 12:	Did the authors of the review account for quality of individual studies when interpreting/ discussing the results of the review?}
A review should take the quality of the individual studies into account when interpreting the results. This will increase the confidence in the findings and conclusions of the review.

To rate 'Yes', appraisers should see that either the review has excluded studies that do not meet the quality criteria defined in the study, or the analysis and conclusions are separated based on the quality of the included studies. The information on using the quality of studies while interpreting the results is expected to be described in the discussion or analysis sections of the review report where results are further discussed/analyzed to draw conclusions.
\newline

\noindent \textbf{Item 13:	Did the authors of the review account for primary studies’ characteristics when interpreting/discussing the results of the review?}
There are many factors that can cause heterogeneity in the results of the included studies. It is important to analyze the causes of the heterogeneity in results, if any, while interpreting the results and drawing any conclusions. For example, it could be the variations in the contextual factors (e.g., student versus practitioners as subjects) that lead to differences in the results of different studies. Furthermore, quality scores or some specific quality criteria might also help in explaining the heterogeneity observed in the results \cite{kitchenham2015evidence}. This item is concerned with the use of study characteristics in item 8.

In order to rate 'Yes', appraisers should see that the authors of the review have investigated the impact of study characteristics on the findings of the review.

This discussion is likely to be found after the results section of the review report.
\newline

\noindent \textbf{Item 14:	Did the authors of the review provide appropriate recommendations and conclusions from the review?}
The usefulness of results of the review for the target stakeholders is critical to assess the relevance of the review. This item is a reflection on the aims as motivation for the review assessed in the first item of the instrument (i.e., item 1).

For `Partial Yes' the review should have satisfactory recommendations and conclusions based on the review results. 

For `Yes' the recommendations and conclusions from the review shall be traceable to the review results, clearly targeting specific stakeholders, well aligned with the motivation and provides new insights to the community.

\noindent \textbf{Item 15:	Did the authors of the review report their own potential sources of conflict of interest, including any funding they received for conducting the review?}
To ensure the reliability of a review, it is important that the authors of the review report their sources of funding and any other conflicts of interest. The disclosure of the sources of funding is quite obvious. However, identifying other types of conflicts of interest is not that straightforward. 

For example, if the authors of the review have published on the topic of the review or have a vested interest in the outcome of the review, there is a potential for bias when selecting, analyzing and interpreting their own work and studies with competing alternatives. 

It is encouraged that authors of the review should be experts in the topic area, so it is common that they have published extensively in the topic area. Thus, it is important that the authors of the review document report their effort in identifying any conflicts of interest they have, which is relevant for the review. A mitigation strategy in this case is to establish a protocol and have it reviewed by independent researchers not participating in the literature review.

To rate 'Yes', the appraisers should ensure that the authors of the review have reported on the presence or absence of any conflicts of interest. In case there was some conflict of interest, the authors of the review should have described and justified the steps taken to mitigate the threat of bias in the results of the review.


==> Critical appraisal of SE SLRs (Paper)(1)/QAISER.tex <==
% %\todo{IMPORTANT: discuss what we want to specify regarding inter-rater agreement and acceptable levels in items about selection, extraction and quality assessment 5,6, 10} ,DONE
% %\todo{IMPORTANT: review the instrument and where possible introduce where pilot was done.} DONE!!
\onecolumn
\section*{Appendix A. QAISER instrument}
\label{AppendixA}
% %\todo{Introduction: Explain the order of the questions and how they are grouped (as discussed at our meeting). Introduce the target users, scope, purpose of QAISER and how it can be used. Also introduce the possibility to use expert judgement in the evaluation. Consult the guidance doc especially when using QAISER initially, which ought to include examples.}

% \subsection{QAISER Instrument: item level assessment}
% QAISER's items and responses are presented in Table \ref{tab:QAISER}.

% %\end{landscape}

% % \paragraph{Group level assessment}: We organized the 15 QAISER items into seven groups (see first column in Table \ref{tab:groups}) corresponding to the process and outcome of an SLR. Having completed the assessment of individual items above, an appraiser should reflect on the impact of the weaknesses on the reliability and relevance of the SLR at the group level. Groups 1, 2, 6, and 7 consist of single items only, and are therefore relatively simple to reflect upon. A ''No'' rating on the corresponding items of these four groups indicates a major weakness at the group level. Groups 3, 4, and 5 consist of multiple items and are more complex to reflect upon. The appraisers should make an overall assessment after considering the ratings of all items in the groups. As a rule of thumb, we recommend that all items receiving a ``No'' should be considered as hinting at a major weakness in the group being assessed.

% % \paragraph{SLR level assessment}: Once the reflection on the group level is complete, an appraiser should use it to provide the assessment about the following two aspects at the SLR level:

% % \begin{enumerate}
% %     \item Reliability of an SLR: The reliability of an SLR is assessed by rating the overall confidence in the results of an SLR as: high, moderate, low or critically low. Apart from group 1, all other groups are relevant while considering the confidence in the results of an SLR. As a rule of thumb, we recommend that the confidence in the SLRs with major weaknesses in groups 3, 4 and 5 should be considered ``critically low''.
% %     %While major weaknesses in groups 2 and 6 along with major weaknesses in at most two of the groups 3, 4, 5 should be considered ``low''. 
% %     %We recommend that any SLR with major weaknesses in either group 2 or group 6 and no major weaknesses in groups 3, 4, 5 and 7 should be judged as having moderate confidence. Finally, a review with a few or no weaknesses in groups 3, 4, 5 and 7 and only a few minor weaknesses in 2 and 6 should be considered an SLR with high confidence in results. 
% %     Table \ref{tab:Reliability} provides guidance for interpreting weaknesses observed at the group level to select a confidence rating at the SLR level.
    
% %     \item Relevance of an SLR: The relevance of an SLR is also rated as high, moderate, low or critically low. Groups 1 and 6 are relevant when making a judgement about the relevance of an SLR. As a rule of thumb, we recommend that the relevance of an SLR be judged to be ``critically low'' if there are major weaknesses in both groups 1 and 6. Table \ref{tab:Relevance} provides guidance in selecting a relevance rating based on the weaknesses in groups 1 and 6.
% % \end{enumerate}

% % The guidance provided in Table \ref{tab:Reliability} and \ref{tab:Relevance} is one recommendation. The appraisers can and should decide which groups of items are more/less critical for the specific review being assessed.


%\onecolumn

\begin{longtable}{p{7cm}p{8cm}p{1.9cm}}
	\caption{QAISER Instrument.}\\
	\label{tab:QAISER}
	 &  &  \\
	\endfirsthead
	%
	\multicolumn{3}{c}%
	{{\bfseries Table \thetable\ continued from previous page}} \\
	 &  &  \\
	\endhead
	%
	\toprule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{1.     Did the authors of the review adequately justify the need for undertaking the review? \cite{kitchenham2015evidence,PETERSEN20151,AMPATZOGLOU2019201}}} \\
	\midrule
	For Partial Yes: & For Yes: &  \\
	\midrule
    The authors of the review should have: &  As for partial yes, plus the authors of the review should also have ALL of the following:\\
	\midrule
	{$\square$} Identified existing related reviews on the topic, or explained that no related review exists.\newline
	&
	{$\square$} Discussed related existing reviews on the topic, if any. \newline
	{$\square$} Established a scientific or practical need for their review \cite{kitchenham2015evidence}.
	\newline &
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	\midrule
	Comments:&\\
	&&\\
	\midrule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{2.     Did the authors of the review establish a protocol prior to the conduct of the review? \cite{Sheaj4008,AMPATZOGLOU2019201,kitchenham2015evidence}}} \\
	\midrule
	For Partial Yes: & For Yes: &  \\
	\midrule
    The authors of the review state that they had a written protocol that is publicly available that should specify ALL of the following: & As for partial yes, plus ALL of the following: &  \\
	\midrule
	{$\square$} Appropriate review questions \cite{Sheaj4008,kitchenham2015evidence,PETERSEN20151} \newline
	{$\square$} Search process \cite{Sheaj4008,kitchenham2015evidence} \newline
	{$\square$} Study selection process \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201} \newline
	{$\square$} Data extraction process \cite{kitchenham2015evidence} \newline
	{$\square$} Study quality assessment process \cite{Sheaj4008,kitchenham2015evidence}\newline
	{$\square$} An outline of the data synthesis plan \cite{Sheaj4008,kitchenham2015evidence} &
	{$\square$} The justifications of any deviations from the protocol should be documented \cite{Sheaj4008,AMPATZOGLOU2019201,kitchenham2015evidence}. \newline
	{$\square$} The protocol should have been internally validated by piloting selection criteria, search strings, data extraction and synthesis processes  \cite{kitchenham2015evidence}. \newline
	{$\square$} The protocol should have been validated by an external reviewer \cite{kitchenham2015evidence}. \newline
	
	&
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	\midrule
	Comments:&\\
	&&\\
	\midrule
	\multicolumn{3}{p{16.6cm}}{\textbf{3.     Are the review's inclusion and exclusion criteria appropriate?} } \\
	\midrule
	
	For Yes: the review should have ALL of the following: & &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{$\square$} Reported the inclusion and exclusion criteria \cite{DARE,kitchenham2015evidence,AMPATZOGLOU2019201}.
	\newline
	{$\square$} The criteria are aligned with the review questions. \newline
	{$\square$} Provided appropriate justifications for any restrictions used in the inclusion and exclusion criteria (e.g.,topic-related scoping restrictions, time-frame,  language, study type, and peer reviewed works only) \cite{kitchenham2015evidence,Sheaj4008}.} & 
	{$\square$} Yes \newline
	{$\square$} No \\
	&  &  \\
	\midrule
	Comments:&\\
	&& \\
	\midrule
	\multicolumn{3}{p{16.6cm}}{\textbf{4.     Did the authors of the review use a comprehensive literature search strategy? \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201,DARE} }}  \\
	\midrule
	When database search is used as the main method &  &  \\
	\midrule
	For Partial Yes: & For Yes: &  \\
	\midrule
	The review should have All of the following: & As for partial yes, plus the review should also have used: &  \\
	\midrule
	{$\square$} An appropriate process for constructing the search strings including piloting \cite{kitchenham2015evidence,AMPATZOGLOU2019201} \newline
	{$\square$} Search process validation based on an appropriate level of recall and precision using a known-set of papers \cite{kitchenham2015evidence,AMPATZOGLOU2019201,PETERSEN20151}  \newline
	{$\square$} At least one relevant indexing database (e.g., Scopus) in combination with relevant publisher databases (e.g., IEEE and ACM) \cite{kitchenham2015evidence} \newline
	{$\square$} Appropriately documented the search process (e.g., known-set, search strings, and search results) \cite{kitchenham2015evidence,AMPATZOGLOU2019201, AliU18}  & 
	{$\square$} At least one additional search method (e.g., snowballing, manual search, or use DBLP or Google scholar of key researchers) \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201} &
	 {$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	&  &  \\
	\midrule
	When snowballing is used as the main method &  &  \\
	\midrule
	For Partial Yes: & For Yes: &  \\
	\midrule
	The review should have ALL of the following: & As for partial yes, plus the review should also have used either ONE of the following: &  \\
	\midrule
	{$\square$} Appropriately justified the use of snowballing as the main method \cite{kitchenham2015evidence} \newline
	{$\square$} Selected an appropriate start/seed set \cite{Wohlin:2014:GSS:2601248.2601268} \newline
	{$\square$} Performed an acceptable number of backward and forward snowballing iterations \cite{Wohlin:2014:GSS:2601248.2601268} & 
	{$\square$} At least one additional search method (e.g., manual search, or use DBLP or Google scholar of key researchers) \cite{Wohlin:2014:GSS:2601248.2601268,kitchenham2015evidence} \newline
	{$\square$} Snowballing iterations until no new papers were found \cite{Wohlin:2014:GSS:2601248.2601268}&
	 {$\square$} Yes\newline
	 {$\square$} Partial Yes\newline
	 {$\square$} No \\
	 
	 \midrule
	Comments:&\\
	 &  &  \\
	\midrule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{5.     Did the authors of the review use a reliable study selection process? \cite{Sheaj4008,kitchenham2015evidence,PETERSEN20151} }} \\
	\midrule
	
	For Partial Yes: & For Yes, either ONE of the following: &  \\
	\midrule
	{$\square$} At least two authors of the review selected a representative sample of eligible studies and achieved good agreement, with the remainder selected by one review author \cite{Sheaj4008, kitchenham2015evidence, AMPATZOGLOU2019201}. \newline 
	&
	{$\square$} At least two authors of the review independently agreed on selection of eligible studies, reached consensus on which studies to include, and reported the agreement level \cite{Sheaj4008,kitchenham2015evidence,PETERSEN20151}.\newline 
	{$\square$} OR if only a sample of studies were selected by two authors, all excluded studies were reviewed by at least two authors of the review.  \newline
	&
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{6.     Did the authors of the review use a reliable data extraction process? \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201,PETERSEN20151} }} \\
	\midrule
	
	For Partial Yes: & For Yes: &  \\
	\midrule
	{$\square$} At least two authors of the review extracted data from a sample of included studies and achieved good agreement, with the remainder extracted by one review author \cite{Sheaj4008,kitchenham2015evidence,PETERSEN20151} \newline
	&
	{$\square$} At least two authors of the review achieved consensus on which data to extract from the included studies \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201,PETERSEN20151} &
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{7.     Did the authors of the review provide a list of excluded studies, along with the justifications for exclusion, that were read in full text? \cite{Sheaj4008,kitchenham2015evidence} }}\\
	\midrule
	For Partial Yes, the review should have: & For Yes, the review should also have: &  \\
	\midrule
	{$\square$}  Provided a list of all potentially relevant studies that were read in full text, but excluded from the review \cite{Sheaj4008,kitchenham2015evidence} & 
	{$\square$}  Justified the exclusion from the review of each potentially relevant study that was read in full text \cite{Sheaj4008} & 
	{$\square$} Yes\newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&  &  \\
	\midrule
	\multicolumn{3}{p{16.6cm}}{\textbf{8.  Did the authors of the review provide sufficient primary studies' characteristics to interpret the results? \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201,DARE} }}  \\
	\midrule
	For Yes, the review should have described ALL of the following: &  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{{$\square$} Populations \cite{Sheaj4008}\newline	
	{$\square$} Interventions, when applicable \cite{Sheaj4008} \newline
	{$\square$} Outcomes, when applicable \cite{Sheaj4008}\newline
	{$\square$} Study types \cite{Sheaj4008} \newline
	{$\square$} Study contexts \cite{Sheaj4008}}} & 
	{$\square$} Yes\newline{$\square$} No \\
	
	\midrule
	Comments:&\\
	&  &  \\
	\midrule
	\multicolumn{3}{p{16.6cm}}{\textbf{9.     Did the authors of the review use an appropriate instrument for assessing the quality of primary studies that were included in the review? \cite{Sheaj4008,kitchenham2015evidence} }} \\
	\midrule
	\multicolumn{2}{p{16cm}}{For Yes, the review should have used appropriate instruments for different types of studies included in the review. An appropriate instrument would have questions related to ALL of the following \cite{kitchenham2015evidence}: }  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{{$\square$} \textit{"The goals, research questions, hypotheses and outcome measures"} \cite{kitchenham2015evidence}\newline 
	{$\square$} \textit{"The study design and the extent to which it is appropriate to the study type"} \cite{kitchenham2015evidence} \newline
	{$\square$} \textit{"Study data collection and analysis and the extent to which they are appropriate given the study design"} \cite{kitchenham2015evidence} \newline
	{$\square$} \textit{"Study findings, the strength of evidence supporting those findings, the extent to which the findings answer the research questions, and their value to practitioners and researchers"} \cite{kitchenham2015evidence} }}  & 
	{$\square$} Yes\newline
	{$\square$} No \\
			
	\midrule
	Comments:&\\
	&  &  \\
	\midrule
	
	\multicolumn{3}{p{16.6cm}}{\textbf{10.     Did the authors of the review use a reliable quality assessment process? \cite{kitchenham2015evidence} }} \\
	\midrule
	
	For Partial Yes: & For Yes: &  \\
	\midrule
	{$\square$} At least two authors of the review performed quality assessment of a representative sample of eligible studies and achieved good agreement, with the remainder performed by one review author \cite{kitchenham2015evidence} \newline
	&
	{$\square$} At least two authors of the review independently performed quality assessment of eligible studies, reached consensus, and reported the agreement level \cite{kitchenham2015evidence} &
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule
	
	\multicolumn{3}{p{18cm}}{\textbf{11.  Were the primary studies appropriately synthesized? \cite{DARE,kitchenham2015evidence,AMPATZOGLOU2019201,BudgenBDW18}}} \\
	\midrule
	For Yes, the review should have ALL of the following: &  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{$\square$}   Selected an appropriate synthesis method given the review questions and extracted data \cite{kitchenham2015evidence,AMPATZOGLOU2019201,BudgenBDW18}\newline
	{$\square$} Applied the selected synthesis method appropriately \newline
	{$\square$} Provided a clear trace linking the answers of review questions and interpretations to the data from the primary studies } & 
	{$\square$} Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule
	\multicolumn{3}{p{18cm}}{\textbf{12.  Did the authors of the review account for quality of individual studies when interpreting/discussing the results of the review? \cite{Sheaj4008,kitchenham2015evidence,AMPATZOGLOU2019201} }}  \\
	\midrule
	For Yes, either ONE of the following: &  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{$\square$}  Included only high-quality studies \cite{Sheaj4008,kitchenham2015evidence} \newline
	{$\square$}  OR, the authors have categorized the analysis and interpretation of results based on study quality \cite{Sheaj4008,kitchenham2015evidence} }  & 
	{$\square$} Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule
	
	\multicolumn{3}{p{18cm}}{\textbf{13.  Did the authors of the review account for primary studies' characteristics when interpreting/discussing the results of the review?}}  \\
	\midrule
	For Yes, either ONE of the following: &  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{$\square$}  There were no significant similarities or differences to warrant a separate analysis \newline
	{$\square$}  OR, the authors have appropriately accounted for study characteristics and discussed their impact on the review results \cite{Sheaj4008,kitchenham2015evidence} }  & 
	{$\square$} Yes\newline
	{$\square$} No \\
	
	&&\\
	\midrule

	\multicolumn{3}{p{16.6cm}}{\textbf{14.     Did the authors of the review provide appropriate recommendations and conclusions from the review? \cite{BudgenBDW18} }} \\
	\midrule
	
	For Partial Yes, the review should have: & For Yes, the recommendations and conclusions should also be &  \\
	\midrule
	{$\square$} Provided satisfactory recommendations and conclusions based on the review results \newline
	&
	{$\square$} Clearly traceable back to the review results \newline
	{$\square$} Clearly targeting specific stakeholders \newline
	{$\square$} Well aligned with the upfront motivation for undertaking the review, or are any deviations well explained \newline
	{$\square$} Providing new valuable insights to the community \newline
	&
	{$\square$} Yes \newline
	{$\square$} Partial Yes\newline
	{$\square$} No \\
	
	\midrule
	Comments:&\\
	&&\\
	\midrule

	\multicolumn{3}{p{18cm}}{\textbf{15.  Did the authors of the review report their own potential sources of conflict of interest, including any funding they received for conducting the review? \cite{Sheaj4008,kitchenham2015evidence}}}  \\
	\midrule
	For Yes, either ONE of the following: &  &  \\
	\midrule
	\multicolumn{2}{p{16cm}}{{$\square$}   The authors reported no competing interests \newline
	{$\square$}  OR, the authors described their funding sources \cite{Sheaj4008,kitchenham2015evidence} and how they managed potential conflicts of interest \cite{Sheaj4008}}  &
	{$\square$} Yes\newline
	{$\square$} No \\
	\midrule
	Comments:&\\
	\bottomrule
\end{longtable}


